Operational Quantum Frames: An operational approach to quantum reference frames

The quantum reference frames program is based on the idea that reference frames should be treated as quantum physical systems. In this work, we combine these insights with the emphasis on operationality, understood as refraining from introducing into the framework objects not directly related to in principle verifiable probabilities of measurement outcomes, and identifying the setups indistinguishable as such. Based on intuitions from special relativity and gauge theory, we introduce an operational notion of a quantum reference frame -- which is defined as a quantum system equipped with a covariant positive operator-valued measure (POVM) -- and build a framework on the concept of operational equivalence that allows us to enforce operationality by quotienting the quantum state spaces with equivalence relation of indistinguishability by the available effects, assumed to be invariant under gauge transformations, and framed in the sense of respecting the choice of the frame's POVM. Such effects are accessed via the yen construction, which maps effects on the system to those on the composite system, satisfying gauge invariance and framing. They are called relative, and the classes of states indistinguishable by them are referred to as relative states. We show that when the frame is localizable, meaning that it allows for states that give rise to a highly localized probability distribution of the frame's observable, by restricting the relative description upon such localized frame preparation we recover the usual, non-relational formalism of quantum mechanics. We provide a consistent way of translating between different relative descriptions by means of frame-change maps and compare these with the corresponding notions in other approaches to QRF, establishing an operational agreement in the domain of common applicability.

==> Chapters/7.Further.tex <==
\section{Open problems}

\section{Relative observables are invariant and framed}




\subsection{Homogenuous Yen}

\subsection{Generalized integration theory}

\subsection{Convolution theory for POVMs}

\section{Generalizations}

\subsection{Algebraic}

\subsubsection{Probability theory as an extension of logic}
Jaynes, Pavlov \cite{Pavlov22}
von Neumann, who was famously admitted not to believe in a framework based on the Hilbert spaces only three years after the publication of his famous work on the subject 

It then seems most natural to treat the predual space of an abstract $W^*$-algebra $\mathcal{N}$, denoted by $\mathcal{N}_\bigstar$, as the home for states in the abstract setting, i.e. without invoking a Hilbert space representation~$\mathcal{N'} \subseteq B(\his)$, generalizing the full space of trace-class operators $\mathcal{T}(\his)$.

\begin{itemize}
    \item positivity
    \item normalization
    \item Hilbert space less definition of states
\end{itemize}

\subsection{Convex-theoretic}


\section{Relational emergence}



\subsection{Relationality of Measurement}\label{measuringY}

\jan{I just put it here for now, nothing hangs on it}
An experimental setup for the measurement of a POVM $\E_\S: \mathcal{B}(\Sigma_\S) \to B(\his)$ on a system $\S$ can be described by specifying a measuring apparatus $\R$, which is a quantum system with a Hilbert spaces that we denote by $\hir$, together with a \emph{pointer observable POVM} $\E_\R: \mathcal{B}(\Sigma_\R) \to B(\hir)$ on a sample space $\Sigma_\R$, a \emph{Borel map} $f: \Sigma_\R \to \Sigma_\S$, and a \emph{pointer state} $\omega_p \in \S(\hir)$. Such a setup can be depicted~as

\begin{center}
    \begin{equation}\label{qmsetup}
    \begin{tikzcd}
        B(\hir)                                   & B(\his)                                                       \\
        \mathcal{B}(\Sigma_\R) \arrow[u, "\E_\R"] & \mathcal{B}(\Sigma_\S) \arrow[l, "f^{-1}"] \arrow[u, "\E_\S"].
    \end{tikzcd}
    \end{equation}
\end{center}

Further, an \emph{interaction} between $\R$ and $\S$, i.e. a short time unitary evolution $U_{\Delta t} = e^{iH\Delta t} \in B(\hir \otimes \his)$, is introduced that entangles an initially separable state $\omega_p \otimes \rho \in \S(\hir \otimes \his)$ in a way that allows to recover the measurement statistics of $\E_\S$ on $\rho$ by measuring the pointer observable $\E_\R$, i.e. for any $X \in \mathcal{B}(\Sigma_\S)$
we should have the \emph{probability reproducibility condition} (PRC) \cite{loveridge2012quantum}:

\begin{equation}\label{probrepcond}
    \tr[U_{\Delta t}^*(\omega_p \otimes \rho)U_{\Delta t}\E_\R(f^{-1}(X)) \otimes \text{Id}_\S ] = \tr[\rho \E_\S(X)]
\end{equation}

Thus the interaction between the system and the measuring apparatus allows an experimenter to access the measurement statistics of the observable $\E_\S$ while the Borel function $f$ allows to relate the sample space $\Sigma_\S$, which is an abstract space, e.g. the spectrum of a self-adjoint operator, with the space $\Sigma_\R$ to which the experimenter has direct access to, e.g.~a~detection screen. One can also see the equation above as defining the observable $\E_\S$ 
by the measurement setup~($U_{\Delta t}$,~$f$,~$\E_\R$,~$\omega_p$). If we now assume, which is a common practice, both sample spaces to be identical and set $f=\text{Id}_\Sigma$, the PRC can be then rewritten in the following form

\[
\tr[(\omega_p \otimes \rho) E_{\R}(\Delta t)(X)] = \tr[\rho \E_\S(X)],
\]

where we have introduced the notation for the evolved frame observable

\[
\E_{\R}(\Delta t) := U_{\Delta t}[\E_\R(\cdot) \otimes \text{Id}_\S]U_{\Delta t}^*.
\]

In the presence of symmetries, i.e. when we have an action of $G$ on $\Sigma_\R$, we should have a corresponding action of $G$ on $\hir$ making $\E_\R$ covariant. A short calculation shows that if the interaction $U_{\Delta t}$ commute with frame 'rotations', i.e. $[U_{\Delta t},U_\R(g) \otimes \text{Id}_{\S}]$ for all $g \in G$, a stronger condition holds. Indeed, for any $h \in G$ we then have

\[
\tr[(h.\omega_p \otimes \rho) E_{\R}(\Delta t)(h.X)] = \tr[\rho \E_\S(X)].
\]

Thus when we 'rotate' the sample space of the apparatus by $h \in G$, which corresponds to acting with $h$ on the $\epsilon$-pointer state, to reproduce the statistics of $\E_\S$ by measuring $E_{\R}(\Delta t)$ on the product state we need to first 'rotate' the input accordingly. We will refer to the above as the \emph{relational reproducibility condition} (RRC). If we further assume that both systems are principal quantum reference frames on the same group $G$, so that $\E_S$ is now assumed covariant as well, and that $\E_\R$ is localizable, for given $\E_S$ and $\E_R$ we can generate the relative orientation observable that will satisfy the RRC in the localized limit. Indeed, take $\omega_n$ to be a localizing sequence for $\E_\R$. Then for any $X \in \mathcal{B}(G)$ we have

\begin{align*}
\lim_{n \to \infty}\tr[(h.\omega_n \otimes \rho) \E_\S*\E_\R (h.X)] &= 
\lim_{n \to \infty}\int_G d\mu_{h.\omega_n}^{\E_\R}(g)\tr[\rho g.\E_\S(hX)]\\ &=
\tr[\rho h^{-1}.\E_\S(hX)] = \tr[\rho \E_\S(X)].
\end{align*}

If we thus localize the frame at $h\in G$, i.e. take the input state to be $(h^{-1}.\omega_n \otimes \rho)$, to reproduce the statistics of $\E_\S$ by measuring $\E_\S*\E_\R$ on the product state we need to first 'rotate' the input set the \emph{opposite} way. This is an instance of an \emph{active} transformation of the frame -- we localize it at a given point in $G$ -- in contrast to the \emph{passive} transformation that we had before, when the whole sample space was being 'rotated'. Given a localizable frame, measuring \emph{any} covariant observable can thus be modeled by a measurement of the corresponding relative orientation observable.

==> Chapters/OperatorAlg.tex <==

\subsection{$C^*$-algebras}

An abstract mathematical object mimicking most of the structure of $B(\his)$ is that of a $C^*$-algebra.

\begin{definition}
    A Banach space $\mathcal{A}$ is a $C^*$-algebra if it is equipped with the operations
    \begin{itemize}
        \item (multiplication) $\cdot: \mathcal{A} \times \mathcal{A} \to \mathcal{A}$ and
        \item (involution) $(\_)^*: \mathcal{A} \to \mathcal{A}$
    \end{itemize}
    satisfying the following compatibility requirements for all $A,B \in \mathcal{A}$
    \begin{enumerate}
        \item $||AB||\leq||A||||B||$,
        \item $(A^*)^*=A$,
        \item $(A+B)^* = A^* + B^*$,
        \item $(AB)^*=B^*A^*$,
        \item $(\lambda A)^*=\overline{\lambda}A^*$,
        \item $||A^*A||=||A||||A^*||$.
    \end{enumerate}
\end{definition}

One can verify that indeed $B(\his)$ is a $C^*$-algebra. A subset $\mathcal{A} \subset B(\his)$ that is closed under multiplication meaning that multiplying a pair of elements from $\mathcal{A}$ does not lead outside of $\mathcal{A}$, is called a subalgebra (of $B(\his)$). It is a $*$-subalgebra if also the involution operation restricts to $\mathcal{A}$, and a Banach space if it is complete as a metric space with the norm inherited from $B(\his)$. The last property is usually referred to as $\mathcal{A}$ being \emph{norm-closed}, since it is equivalent to being a closed subset in the sense of the topology on $B(\his)$ generated by open balls in the sense of the metric $d(A,B)=||B-A||$.\footnote{We will avoid general topological notions and only speak about subsets being closed in the sense of including limits of particular classes of sequences. This is all we actually need and we find this way of thinking to be more easily motivated operationally (see \emph{operational topology} below).} Any norm-closed $*$-subalgebra of $B(\his)$ is also a $C^*$-algebra of its own, and as it turns out it is also the most general kind of a $C^*$-algebra. Indeed, one can show that every $C^*$-algebra is \emph{isomorphic} to such a subalgebra for some (non-unique) Hilbert space $\his$ (the "$C$" coming from "closed"). By isomorphic here we mean that there is a map $\pi:\mathcal{A} \to \mathcal{A'} \subseteq B(\his)$ that is invertible and preserves all the structure, i.e. in this case $\pi$ needs to be a linear bounded map that is isometric and preserves involution in that $||\pi(a)||' = ||a||$ and  $\pi(a^*)=\pi(a)^*$ for any $a \in \mathcal{A}$. We say that any $C^*$-algebra can be \emph{represented} as a $C^*$-subalgebra of some $B(\his)$.

\subsection{$W^*$-algebras}

Mathematically speaking, the states on $C^*$-algebras are defined to be linear functionals $\omega: \mathcal{A} \to \mathbb{C}$ satisfying some extra properties that allow for their usual probabilistic interpretation. Here we will argue that both mathematically and conceptually the reversed relationship is more adequate when it comes to quantum physics -- we would like to treat operators, or elements of $C^*$-algebras, as elements of the space dual to the one in which the states live. As we will shortly see, this perspective perfectly aligns with both the standard Hilbert space-based setting and the operational philosophy as expressed in the form of the so-called Generalized Probabilistic Theories.

 Pure states are characterized among the density operators as one-dimensional projections or as the extreme points, i.e. those elements that can not be written as linear combinations of others, of the convex set $\S(\his)$ of density matrices. We then see that the standard quantum mechanical framework can be expressed entirely in terms of the algebra $B(\his)$, without the need of ever invoking the underlying Hilbert space. From this perspective, the Hilbert spaces seem less fundamental in the context of foundations of quantum mechanics than they are usually presented to be.

The $C^*$-algebra $B(\his)$ then has a \emph{predual} space, i.e. it is isomorphic, as a Banach space, to the dual space of some other Banach space. It can be shown that if such a predual exists for a $C^*$-algebra, it is unique, thus characterizing the space of trace-class operators in terms of the $C^*$-algebra $B(\his)$ alone -- it is \emph{the} predual space of $B(\his)$. Let us distinguish a class of $C^*$-algebras that share this property.

\begin{definition}
    A $C^*$-algebra that admits a predual Banach space is called a $W^*$-algebra.
\end{definition}

Consider now a $W^*$-algebras $\mathcal{N}$ and notice the following. It is a $C^*$-algebras, so we already know that it can be represented as closed $*$-subalgebras $\mathcal{N'} \subseteq B(\his)$ for some Hilbert space $\his$. As it turns out, those algebras can be distinguished from general $C^*$-subalgebras of $B(\his)$ as the ones satisfying a stronger kind of completeness requirement.

\begin{definition}
    A von Neumann algebra is a $C^*$-subalgebra $\mathcal{N'} \subseteq B(\his)$ that contains the identity and is weakly closed.
\end{definition}

The \emph{weak closedness} requirement means that if we have a sequence of operators $\{A_0,A_1,\dots\}$ in a $C^*$-subalgebra $\mathcal{N'} \subseteq B(\his)$ such that for any trace-class operator $\Omega \in \mathcal{T}(\his)$ the sequence of expectation values $\lambda_n^\Omega = \tr[\Omega A_n]$ converges in $\mathbb{C}$, the operator $A_\infty \in \mathcal{N}$ for which $\tr[\Omega A_\infty] = \lim_{n \to \infty} \lambda_n^\Omega$ for all $\Omega \in \mathcal{T}(\his)$, which always exists in $B(\his)$, is contained in $\mathcal{N'}$. Such a sequence of operators is called \emph{weakly convergent}.

The unique predual space is then given by the space of \emph{normal functionals}, which are functionals $\varphi: \mathcal{N'} \to \mathbb{C}$ that are not only bounded but continuous in the following sense: for any weakly converging sequence $\lim_{n \to \infty} A_n = A_\infty$ of operators in $\mathcal{N'}$ we have $\lim_{n \to  \infty} \varphi(A_n) = \varphi(A_\infty)$. In the case of $B(\his)$, the only such functionals are given by trace-class operators via $\phi_{\Omega}: A \mapsto \tr[\Omega A]$ with $\Omega \in \mathcal{T}(\his)$, which is in agreement with our previous characterization of $\mathcal{T}(\his)$ as the predual space of $B(\his)$. In general, those are simply the functionals that come as restrictions of $B(\his) \ni A \mapsto \tr[\Omega A] \in \mathbb{C}$ with $\Omega \in \mathcal{T}(\his)$. The predual $\mathcal{N'}_\bigstar$ of a von Neumann algebra $\mathcal{N'} \subseteq B(\his)$ can then be described as the quotient space
\[
    \mathcal{N'}_\bigstar \cong \mathcal{T}(\his)/\hspace{-3pt}\sim_{\mathcal{N'}},
\]
where $\Omega \sim_{\mathcal{N'}} \Omega'$ if they agree as functionals on $\mathcal{N'}$, i.e. if $\tr[\Omega A] = \tr[\Omega' A]$ for all $A \in B(\his)$. This can be seen as an instance of \emph{operational equivalence} with respect to $\Eff(\mathcal{N})$.



